Finding Alignments Between Interpretable Causal Variables and Distributed Neural Representations

Causal abstraction is a promising theoretical framework for explainable artificial intelligence that defines when an interpretable high-level causal model is a faithful simplification of a low-level deep learning system. However, existing causal abstraction methods have two major limitations: they require a brute-force search over alignments between the high-level model and the low-level one, and they presuppose that variables in the high-level model will align with disjoint sets of neurons in the low-level one. In this paper, we present distributed alignment search (DAS), which overcomes these limitations. In DAS, we find the alignment between high-level and low-level models using gradient descent rather than conducting a brute-force search, and we allow individual neurons to play multiple distinct roles by analyzing representations in non-standard bases-distributed representations. Our experiments show that DAS can discover internal structure that prior approaches miss. Overall, DAS removes previous obstacles to conducting causal abstraction analyses and allows us to find conceptual structure in trained neural nets.

==> arithmeticsection.tex <==
\section{Arithmetic Distribution Rule Experiment}
In our second experiment, we analyze a feed-forward neural network trained to perform a simple arithmetic task where the inputs are three integers $x$, $y$, and $z$ and the output is $(x+y) \cdot z$. Each example in our dataset contains triplets of three integers ranging from 1 to 6, resulting in 38 different outcomes. For simplicity, we cast this task as a classification problem.

\paragraph{Low-Level Neural Model}
We train a multilayer perceptron with a classification head to perform the hierarchical equality task. We concatenate the learned embedding for each digit before passing through the feedforward layers. 

\input{tables/nli-results.tex}

\paragraph{High-Level Models}
In contrast to the hierarchical equality task, there are two oracle high-level causal models that solve this arithmetic task. One model adds the values $x$ and $y$ and then multiplies the sum by $z$. The other model multiplies $x$ by $z$, then multiplies $y$ by $z$, and then adds the two products. The second solution leverages the fact that multiplication distributes over addition. Besides two oracle models, we have two additional high-level models where we only abstract $(x+y)$ or the identity of $y$ as an intermediate variable. 

\paragraph{Results} Our results are shown in \Tabref{tab:arithmeticresults}. The high-level model with addition first reaches the highest \intaccmetricabbr\ compared to others while being far from 100\%. Our results suggest that the high-level model is an \emph{approximate} abstraction of the low-level model. Interestingly, our last high-level model with multiplication first has the lowest \intaccmetricabbr{}. Our findings demonstrate that our neural model is in favor of implementing addition first. 


==> figures/BigMainFig.tex <==

\begin{tikzpicture}[thick,scale=0.6, every node/.style={scale=0.6}]
\def\scalex{3.5}
\def\scaley{1.95}
\def\opac{0.2}
\Large
\def\startx{-17}
\def\starty{7}


\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley+ \starty) {};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty) {$0.53$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley + \starty) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley+ \starty) {$0.23$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley+ \starty) {$-0.09$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley+ \starty) {$0.23$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley+ \starty){$0.68$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley+ \starty){$0.32$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley+ \starty){$0.36$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley+ \starty){$0.68$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley+ \starty){$0.32$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}


\def\startx{0}
\def\starty{7}


\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley+ \starty) {};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty) {$0.5$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley + \starty) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley+ \starty) {$0.91$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley+ \starty) {$-0.09$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley+ \starty) {$-0.09$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley+ \starty){$0$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}




\def\opac{1.0}



\def\scalex{3.5}
\def\scaley{1.95}
\def\opac{0.2}
\Large

\def\startx{17}




\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley+ \starty) {};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty) {$0.06$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley+ \starty) {$0.23$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley+ \starty) {$0.23$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley+ \starty) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley+ \starty) {$-0.09$};


\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley+ \starty){$1$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley+ \starty){$1$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley+ \starty){$1$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}


\def\scalex{3.5}
\def\opac{0.2}
\Large
\def\startx{-17}
\def\starty{-1}

\node[draw, ellipse,  minimum width=180pt, minimum height=44pt] (pi3V1) at ( 0.5 * \scalex+ \startx,1.25 * \scaley + \starty-0.5) {};

\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley+ \starty) {};


\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty) {$0.53$};


\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley + \starty) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley+ \starty) {$0.23$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley+ \starty) {$-0.09$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley+ \starty) {$0.23$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley+ \starty){$0.48$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley+ \starty){$-0.48$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley+ \starty){$0.23$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley+ \starty){$0.23$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley+ \starty){$0.36$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley+ \starty){$0.68$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley+ \starty){$0.32$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}


\def\startx{0}


\def\starty{-1}

\node[draw, ellipse,  minimum width=180pt, minimum height=44pt] (piV1) at ( 2.5 * \scalex+ \startx,1.25 * \scaley + \starty-0.5) {};

\node[draw, ellipse,  minimum width=180pt, minimum height=44pt] (piV2) at ( 0.5 * \scalex+ \startx,1.25 * \scaley + \starty-0.5) {};

\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley+ \starty) {};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty) {$0.5$};

\node(anchor1) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty+ 2) {};

\node(anchor2) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty + 0.4) {};

\draw[->, line width=1mm] (anchor1) -- (anchor2);

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley+ \starty) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley+ \starty) {$0.91$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley+ \starty) {$-0.09$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley+ \starty) {$-0.09$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley+ \starty){$0.48$};

\node[fill=purple!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley+ \starty){$-0.48$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley+ \starty){$0.71$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley+ \starty){$-0.71$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley+ \starty){ $0.32$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley+ \starty){$0.68$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley+ \starty){$0.32$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}




\def\starty{8.54}
\def\opac{1.0}



\def\scalex{3.5}
\def\scaley{1.95}
\def\opac{0.2}
\Large

\def\startx{17}
\def\starty{-1}

\node[draw, ellipse,  minimum width=180pt, minimum height=44pt] (pi2V1) at ( 2.5 * \scalex+ \startx,1.25 * \scaley + \starty-0.5) {};

\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley+ \starty) {};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty) {$0.06$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley+ \starty) {$0.23$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley+ \starty) {$0.23$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley+ \starty) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley+ \starty) {$-0.09$};


\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley+ \starty){$-0.71$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley+ \starty){$0.71$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley+ \starty){$1$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley+ \starty){$1$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}






\draw[dashed, ->, thick] (pi2V1) to[out=165, in=15] (piV1);

\draw[dashed, ->, thick] (pi3V1) to[out=15, in=165] (piV2);


\def\startx{0}


\def\starty{-8}


\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley+ \starty) {};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty) {$0.54$};

\node(anchor1) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty+ 2) {};

\node(anchor2) at (1.5 * \scalex+ \startx,2.75 * \scaley+ \starty + 0.4) {};

\draw[->, line width=1mm] (anchor1) -- (anchor2);

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley+ \starty) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley+ \starty) {$0.91$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley+ \starty) {$-0.09$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley+ \starty) {$-0.09$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley+ \starty){$0.68$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley+ \starty){$0$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley+ \starty){$1$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley+ \starty){$0$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley+ \starty){ $0.32$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley+ \starty){$0.68$};

\node[fill=brown!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley+ \starty){$0.32$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}


\end{tikzpicture}


==> figures/InterchangeIntervention.tex <==

\begin{tikzpicture}[thick,scale=0.6, every node/.style={scale=0.6}]
\def\scalex{3.5}
\def\scaley{1.8}
\def\opac{0.2}
\Large

\def\startx{0}
\def\starty{-1}


\def\starty{-0.5}

\node[draw, ellipse,  minimum width=180pt, minimum height=44pt] (piV1) at ( 2.5 * \scalex+ \startx,1.25 * \scaley + \starty) {};

\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley) {\Huge $\texttt{False}$};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley) {\Large $0.3775$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley) {$0.23$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley) {$0.23$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley) {$-0.09$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley){$0$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley){$1$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley){$0$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley){$1$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley){$1$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}



\def\startx{0}

\def\scaley{3}


\def\scalex{3.5}
\def\scaley{2}


\def\starty{8}



    



\node[fill=green!20, draw, circle, minimum size=40pt] (A) at (0+ \startx,0+ \starty) {};

\node[fill=green!20, draw, circle, minimum size=40pt] (B) at (1*\scalex+ \startx,0+ \starty) {};

\node[fill=green!20, draw, circle, minimum size=40pt] (C) at (2*\scalex+ \startx,0+ \starty) {};

\node[fill=green!20, draw, circle, minimum size=40pt] (D) at (3*\scalex+ \startx,0+ \starty) {};


\node[fill=blue!20, draw, ellipse, minimum size=20pt] (E) at (0.5*\scalex+ \startx,0.5*\scaley+ \starty) {\texttt{True}};



\node[fill=blue!20, draw, ellipse, minimum size=20pt] (F) at (2.5*\scalex + \startx,0.5*\scaley+ \starty) {\texttt{False}};



\node[fill=yellow!20, draw, ellipse, minimum size=20pt] (G) at (1.5*\scalex + \startx,1*\scaley+ \starty) {\texttt{False}};




\def\starty{8.54}
\def\opac{1.0}



\foreach \xshift in {0,1}{
    \node[fill=purple!80, draw,regular polygon, regular polygon sides=5, minimum size=10pt] () at (\xshift *\scalex + \startx,-0.3*\scaley+ \starty) {};
}

\foreach \xshift in {2}{
    \node[fill=orange!80, draw,regular polygon, regular polygon sides=3, minimum size=16pt,inner sep=0pt] () at (\xshift *\scalex +  \startx,-0.309*\scaley+ \starty) {};
}

\foreach \xshift in {3}{
    \node[fill=green!80, draw,regular polygon, regular polygon sides=4, minimum size=10pt] () at (\xshift *\scalex + 0*\scalex+ \startx,-0.3*\scaley+ \starty) {};
}






\draw [->,opacity=\opac] (A) -- (E);
\draw [->,opacity=\opac] (B) -- (E);
\draw [->,opacity=\opac] (C) -- (F);
\draw [->,opacity=\opac] (D) -- (F);
\draw [->,opacity=\opac] (E) -- (G);
\draw [->,opacity=\opac] (F) -- (G);









\def\scalex{3.5}
\def\scaley{1.95}
\def\opac{0.2}
\Large

\def\startx{17}
\def\starty{-1}


\def\starty{-0.5}

\node[draw, ellipse,  minimum width=180pt, minimum height=44pt] (pi2V1) at ( 2.5 * \scalex+ \startx,1.25 * \scaley + \starty) {};

\node (label) at (1.5 * \scalex+ \startx,3.25 * \scaley) {\Huge $\texttt{True}$};

\node[fill=yellow!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt](out) at (1.5 * \scalex+ \startx,2.75 * \scaley) {\Large $0.5$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT00) at (0 * \scalex+ \startx,0 * \scaley) {$-0.09$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT01) at (1 * \scalex + \startx,0 * \scaley) {$0.23$};

\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT02) at (2 * \scalex+ \startx,0 * \scaley) {$0.91$};
\node[fill=green!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT03) at (3 * \scalex + \startx,0 * \scaley) {$0.91$};


\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT10) at (0 * \scalex+ \startx,1 * \scaley){$0$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT11) at (1 * \scalex+ \startx,1 * \scaley){$0.32$};

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT12) at (2 * \scalex+ \startx,1 * \scaley){$0$ };

\node[fill=red!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT13) at (3 * \scalex+ \startx,1 * \scaley){$1$ };

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT20) at (0 * \scalex+ \startx,2 * \scaley){$0$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT21) at (1 * \scalex+ \startx,2 * \scaley){$0.68$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT22) at (2 * \scalex+ \startx,2 * \scaley){$0.32$};

\node[fill=blue!20, draw, rectangle, rounded corners=3pt, minimum width=40pt, minimum height=20pt] (BERT23) at (3 * \scalex+ \startx,2 * \scaley){$1.0$};


\foreach \col in {0,1,2,3}{
\foreach \coll in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT0\col.north) to (BERT1\coll.south);
\draw[opacity=0.3, ->] (BERT1\col.north) to (BERT2\coll.south);
}
}


\foreach \col in {0,1,2,3}{
\draw[opacity=0.3, ->] (BERT2\col.north) to (out.south);
}



\def\startx{17}

\def\scaley{3}


\def\scalex{3.5}
\def\scaley{2}

\def\starty{8}



    



\node[fill=green!20, draw, circle, minimum size=40pt] (A) at (0+ \startx,0+ \starty) {};

\node[fill=green!20, draw, circle, minimum size=40pt] (B) at (1*\scalex+ \startx,0+ \starty) {};
    
\node[fill=green!20, draw, circle, minimum size=40pt] (C) at (2*\scalex+ \startx,0+ \starty) {};

\node[fill=green!20, draw, circle, minimum size=40pt] (D) at (3*\scalex+ \startx,0+ \starty) {};


\node[fill=blue!20, draw, ellipse, minimum size=20pt] (E2) at (0.5*\scalex+ \startx,0.5*\scaley+ \starty) {\texttt{False}};



\node[fill=red!20, draw, ellipse, minimum size=20pt] (F2) at (2.5*\scalex + \startx,0.5*\scaley+ \starty) {\texttt{False}};



\node[fill=yellow!20, draw, ellipse, minimum size=20pt] (G) at (1.5*\scalex + \startx,1*\scaley+ \starty) {\texttt{True}};

\def\starty{8.54}
\def\opac{1.0}

\foreach \xshift in {0}{
    \node[fill=green!80, draw,regular polygon, regular polygon sides=4, minimum size=10pt] () at (\xshift *\scalex + 0*\scalex+ \startx,-0.3*\scaley+ \starty) {};
}

\foreach \xshift in {1}{
    \node[fill=purple!80, draw,regular polygon, regular polygon sides=5, minimum size=10pt] () at (\xshift *\scalex + \startx,-0.3*\scaley+ \starty) {};
}

\foreach \xshift in {2,3}{
    \node[fill=orange!80, draw,regular polygon, regular polygon sides=3, minimum size=16pt,inner sep=0pt] () at (\xshift *\scalex +  \startx,-0.309*\scaley+ \starty) {};
}







\draw [->,opacity=\opac] (A) -- (E2);
\draw [->,opacity=\opac] (B) -- (E2);
\draw [->,opacity=\opac] (C) -- (F2);
\draw [->,opacity=\opac] (D) -- (F2);
\draw [->,opacity=\opac] (E2) -- (G);
\draw [->,opacity=\opac] (F2) -- (G);



\draw[dashed,  ->, thick] (F) to[out=7, in=173] (F2);
\draw[dashed, ->, thick] (piV1) to[out=15, in=165] (pi2V1);


\end{tikzpicture}


==> intro-alt.tex <==
When can a complex neural network model be said to implement a higher-level algorithm? This is a key question for explainable AI; a positive answer can provide guarantees about how the model will behave, and a negative answer could lead to fundamental concerns about whether the model will be safe and trustworthy for all inputs.  

Causal abstraction provides a mathematical framework for precisely characterizing what it means for any complex causal system (e.g., a deep learning model) to implement a simpler causal system (e.g., a symbolic algorithm), and for assessing whether this relationship holds in practice for modern AI models.  The fundamental operation is the \textit{interchange intervention}, in which a neural network is provided a `base' input and sets of neurons are forced to take on the values they would have if a different `source' input were processed. \citet{Geiger:2021} show that the causal abstraction relation obtains when interchange interventions on aligned high-level variables and low-level variables have equivalent effects. These techniques have been applied to diverse problems \cite{Geiger-etal:2019,Geiger-etal-2020,Li2021,Huang-etal:2022}, and \citet{geigericard} establish formal relationships to a wide range of recent intervention-based analysis methods \citep{vig2020causal,Csordas2021,CausalLM,Ravfogel:2020, Elazar-etal-2020,de2021sparse,abraham-etal-2022-cebab,olah2020zoom,olsson2022context}.

However, previous applications of causal abstraction have faced two central challenges. First, causal abstraction requires a computationally intensive brute-force search process to find optimal alignments between the variables in the high-level model and the states of the low-level one. Where exhaustive search is intractable, we risk missing the best alignment entirely. Second, these prior methods artificially limit the space of possible alignments, by presupposing that high-level causal variables will be aligned with disjoint groups of neurons. There is no reason to assume this a priori, and indeed much recent work in model explanation (see especially \citealt{olah2020zoom,olsson2022context}) is converging on the insight of \citet{Smolensky1986},  \citet{PDP1}, and \citet{PDP2} that individual neurons can play multiple conceptual roles.

With the current paper, we propose \methodname\ (\methodabbr), which overcomes the above limitations of prior causal abstraction work. In \methodabbr, we learn the best alignment via gradient descent rather than having to explore all possible alignments by enumeration, and the alignments involve what \citet{Smolensky1986} called ``patterns'', i.e.,  linear combinations of unit coordinate vectors, rather than being restricted to local sets of pre-specified neurons. The core of \citeauthor{Smolensky1986}'s proposal is that changing the basis for a vector of neurons can better reveal how concepts are represented, and \methodabbr\ makes good on this.

Our experiments involve three distinct tasks. These experiments seek to evaluate \methodabbr\ as an evaluation method, and to substantiate a number of specific claims about the analytic value of \methodabbr\ for explainable AI.  Thus, we work with synthetic tasks that allow us to reason confidently about the explanations \methodabbr\ can offer as compared to standard causal abstraction.

We begin with a case in which standard causal abstraction techniques fail to find a correct alignment but  \methodabbr\  succeeds in doing so. The task is a hierarchical equality task that has been used extensively in developmental and cognitive psychology as a test of relational reasoning: the inputs are sequences $[w, x, y, z]$, and the label is given by $(w=x) = (y=z)$. We train a simple feed-forward neural network on this task and show that it perfectly solves the task. Our key question: does this model implement a program that computes $w=x$ and $y=z$ as intermediate values, as we might hypothesize humans do? Using \methodabbr, we find such an alignment: this high-level model is thus a perfect abstraction of the network. In contrast, standard causal abstraction techniques fail to support this alignment, thus leading us to a spurious negative conclusion about the nature of the model's solution.

Our next set of experiments show that \methodabbr\ can support rigorous comparisons between competing hypotheses about which solution a network has found. We focus on analyzing the representations of numerals in a feed-forward network trained on the arithmetic task $z \cdot (x + y)$. With \methodabbr, we find almost no evidence that the network represents the variables $z \cdot x$ and $z \cdot y$ needed to carry out the algorithm $z \cdot x + z \cdot y$. However, we find substantial (albeit not flawless) evidence of partial abstraction for the computation of $x + y$. This demonstrates the use of \methodabbr\ to adjudicate between alternative explanations, even when neither is perfect.

Finally, we show that \methodabbr\ can avoid a pitfall that prior causal abstraction methods are suceptible to. Our task domain is lexical entailment in a pretrained language model fine-tuned on a natural language inference (NLI) task. With standard causal abstraction, we find an aligment with a simple model of lexical entailment. However, the  \methodabbr\ analysis is more subtle: the distributed representation aligned with the lexical entailment variable can be further decomposed into two representations of the specific lexemes. In other words, what appears to be a representation of lexical entailment is, in this case, a ``data structure'' containing two representations of lexeme identity, rather than an encoding of their entailment relation.

In all of the above experiments, the \methodabbr\ alignment is learned efficiently rather than found by brute-force search. Thus, taken together, the above insights suggest that \methodabbr\ is a more trustworthy, comprehensive, and efficient variant of standard causal abstraction.


==> methods.tex <==
We define an \textbf{acyclic causal model} $\mathcal{M}$ to consist of input, intermediate, and output variables, where each \textbf{variable} has an associated set of \textbf{values} it can take on and a \textbf{causal mechanism} that determine the value of the variable based on the value of its parents. A \textbf{setting} assigns some variables values and is \textbf{total} if it assigns every variable a value, and \textbf{partial} otherwise. \textbf{Input} and \textbf{output} setting are partial settings that assign values to all and only input and output variables, respectively.

An input setting $\mathbf{x}$ of a model $\mathcal{M}$ determines a unique total setting that we denote as $\mathcal{M}(\mathbf{x})$. The inputs are fixed to be $\mathbf{x}$, and then the causal mechanisms of the model determine the values of the remaining variables along the causal structure. We denote the values that  $\mathcal{M}(\mathbf{x})$ assigns to the variables $\mathbf{Y}$ as $\textsc{GetValues}(\mathcal{M}(\mathbf{x}), \mathbf{Y})$.


An intervention $\mathbf{I} \leftarrow \mathbf{i}$ is a partial settings $\mathbf{i}$ of variables $\mathbf{I}$. Together, an intervention and an input setting $\mathbf{x}$ of a model $\mathcal{M}$ determine a unique total setting that we denote as $\mathcal{M}_{\mathbf{I} \leftarrow \mathbf{i}}(\mathbf{x})$.  The inputs are fixed to be $\mathbf{x}$, and then the causal mechanisms of the model determine the values of the non-intervened variables along the causal structure, with the intervened variables $\mathbf{I}$ being fixed to $\mathbf{i}$.



Causal models allow us to formalize symbolic algorithms and neural networks in a common language. Abstraction will allow us to formalize the exact properties a neural network must have to implement a symbolic algorithm.

\begin{definition}{\textnormal{Alignments between Causal Models}}
We define an \textbf{alignment} ($\Pi$, $\tau$) between a low-level causal model $\mathcal{L}$ and high-level causal model $\mathcal{H}$ to be an assignment to each high-level variable $X$ a set of low-level variables $\Pi_{X}$, and a function $\tau_X$ that maps from values of the low-level variables in $\Pi_X$ to values of the aligned high-level variable $X$. Input, output, and intermediate variables must be aligned across the two models, respectively.
\end{definition}

\begin{definition}{\textnormal{Constructive Abstraction}}
A high-level causal model $\mathcal{H}$ is a constructive abstraction of a low-level causal model $\mathcal{L}$ under alignment $(\Pi, \tau)$ exactly when the following holds for every low-level input setting $\mathbf{x}$ and low-level intervention $\mathbf{I} \leftarrow \mathbf{i}$
\[ \tau(\mathcal{L}_{\mathbf{I} \leftarrow \mathbf{i}}(\mathbf{x})\big ) = \mathcal{H}_{\tau(\mathbf{I} \leftarrow \mathbf{i})}(\tau(\mathbf{x}))\]
\end{definition}
When $\mathcal{H}$ is a causal abstraction of $\mathcal{L}$ under an alignment, that guarantees the causal mechanism for each high-level variable $X$ is a faithful simplification of the causal mechanisms for the low-level variables in $\Pi_X$. 

\begin{definition}{\textnormal{Interchange Interventions}}\label{def:intinv}
Given a ``base'' input setting $\mathbf{b}$, ``source'' input settings $\mathbf{s}_1, \dots, \mathbf{s}_k$, and sets of intermediate variables $\mathbf{X}_1, \dots, \mathbf{X}_k$ for causal model $\mathcal{M}$ with output variables $\mathbf{Outputs}$, we define an \textbf{interchange intervention} in two lines, as follows
\[\mathbf{I} \leftarrow \mathbf{i} \;\;\; \overset{\textit{def}}{=}\;\; \bigcup_{1\leq j \leq k} \mathbf{X}_j \leftarrow \bigcup_{1\leq j \leq k} \textsc{GetValues}(\mathcal{M}(\mathbf{s}_j), \mathbf{X}_j)\]
\vspace{-17pt}
\begin{multline*}
\intinv(\mathcal{M}, \mathbf{b}, (\mathbf{s}_1, \mathbf{X}_1), \dots, (\mathbf{s}_k, \mathbf{X}_k)) \overset{\textit{def}}{=} \\
\textsc{GetValues}(\mathcal{M}_{\mathbf{I} \leftarrow \mathbf{i}}, \mathbf{Outputs})
\end{multline*}
\end{definition}

In words, the function $\intinv$ produces the output setting determined by the causal model when provided a base input $\mathbf{b}$ and intervention that fixes variables $\mathbf{X}_1, \dots \mathbf{X}_k$ to be the values they would realize on source inputs $\mathbf{s}_1, \dots \mathbf{s}_k$, respectively.


\begin{definition}{\textnormal{Interchange Intervention Accuracy }}\label{def:intinvacc}
Given low-level and high-level causal models $\mathcal{L}$ and $\mathcal{H}$ with alignment $(\Pi, \tau)$, if we let $\mathbf{Inputs}_L$ be low-level input settings and $\mathbf{Vars}_H$ be high-level intermediate variables the \textbf{interchange intervention accuracy (\intaccmetricabbr)} is as follows
\begin{multline*}
\sum_{\begin{tabular}{c}
      $\mathbf{b},\mathbf{s}_1,\dots, \mathbf{s}_k \in \mathbf{Inputs}_L$\\
      $X_1, \dots, X_k \in \mathbf{Vars}_H$\\
\end{tabular}
      }\\ [\tau\big (\intinv(\mathcal{L}, \mathbf{b},  (\mathbf{s}_1, \Pi_{{X}_1}), \dots, (\mathbf{s}_k, \Pi_{{X}_k}))\big) = \\
      \intinv(\mathcal{H}, \tau(\mathbf{b}),  (\tau(\mathbf{s}_1), {X}_1), \dots, (\tau(\mathbf{s}_k), {X}_k))]
\end{multline*}
\end{definition}


\intaccmetricabbr\ is the proportion of aligned interchange interventions that have equivalent high-level and low-level effects. In our example with $\mathcal{N}$ and $\mathcal{A}$ \intaccmetricabbr\ is 100\% and the high-level model is a perfect abstraction of the low-level model. When \intaccmetricabbr\ is $\alpha<$100\%, we rely on the graded notion of $\alpha$\textit{-on-average} approximate causal abstraction \cite{geigericard}, which directly coincides with \intaccmetricabbr.




\subsection{Rotated Models and Distributed Representations}
An essential aspect of distributed neural representations is that there is a many-to-many mapping between neurons and concepts, meaning that multiple high-level causal variables might be encoded in structures from overlapping groups of neurons \cite{PDP1,PDP2}. In particular, \citet{Smolensky1986} proposes that viewing a neural representation under a basis that is not aligned with individual neurons can reveal the interpretable distributed structure of the neural representations. To make good on this insight, we define a general rotation operator on causal models with variables whose values form a vector space. The result is an identical causal model, except the rotated variables are now expressed on a new basis.

For the following definitions, let $\mathbf{X}$ be an anti-chain\footnote{Antichains are sets of variables where no variable is a causal descendent of any other variable in the set. A layer in a feedforward neural network is a typical example.} %
of variables in $\mathcal{M}$ such that values of $\mathbf{X}$ form a vector space with $|\mathbf{X}|$ dimensions. Let $R_\mathbf{X}$ be an $|\mathbf{X}|$ by $|\mathbf{X}|$ orthogonal matrix from that vector space.

\begin{definition}{\textnormal{Rotated Causal Models}}
 We define the \textbf{rotated causal model} $R_{\mathbf{X}}(\mathcal{M})$ to be identical to $\mathcal{M}$ except the causal mechanisms of $\mathbf{X}$ are modified to rotate the values with $R_{\mathbf{X}}$ and the causal mechanisms that determine the children of $\mathbf{X}$ are modified to rotate the values with $R_{\mathbf{X}}^{-1}$. 
\end{definition}
The representational content of neural activations is at least in part a matter of causal role \cite{block86}. However, ``hard'' interventions fix neurons to constant values, which means they cannot isolate distributed representations expressed in a basis that isn't neuron aligned. In order to characterize the causal role of a distributed representation, we need a ``soft'' intervention that can isolate such basis dimensions by editing causal mechanisms with a rotation, intervention, and then ``unrotation''.  
\begin{definition}{\textnormal{Distributed Interventions}}
A distributed intervention is identified with an orthogonal matrix $\mathbf{R}_{\mathbf{X}}$ and an intervention $\mathbf{I} \leftarrow \mathbf{i}$ where $\mathbf{I} \subseteq \mathbf{X}$. To perform a distributed intervention, simply rotate, interchange intervene, then unrotate $\mathbf{R}_{\mathbf{X}}^{-1}(\mathbf{R}_{\mathbf{X}}(\mathcal{M})_{\mathbf{I} \leftarrow \mathbf{i}})$.
\end{definition}
Interchange interventions are hard interventions, meaning they are limited in their ability to characterize the causal role of distributed neural representations. To address this shortcoming, we extend interchange interventions to target dimensions from a basis that isn't neuron aligned.
\begin{definition}{\textnormal{Distributed Interchange Interventions}}
Begin with a causal model $\mathcal{M}$ with output variables $\mathbf{Outputs}$, a ``base'' input setting $\mathbf{b}$, ``source'' input settings $\mathbf{s}_1, \dots, \mathbf{s}_k$, and sets of intermediate variables $\mathbf{X}_1, \dots, \mathbf{X}_k$ to be intervened upon. Further consider an orthogonal ``rotation'' matrix $\mathbf{R}_{\mathbf{Z}}$ for some set that contains an intervened variable $\mathbf{Z} \cap \bigcup_{1\leq j \leq k}\mathbf{X}_j \neq \emptyset$. We define an \textbf{distributed interchange intervention} as follows. 
\begin{multline*}
\mathbf{I} \leftarrow \mathbf{i} \;\;\; \overset{def}{=}\;\; \bigcup_{1\leq j \leq k} \mathbf{X}_j \leftarrow \bigcup_{1\leq j \leq k} \textsc{GetValues}(\mathcal{M}(\mathbf{s}_j), \mathbf{X}_j)\\
\dintinv(\mathcal{M},\mathbf{R}_{\mathbf{Z}}, \mathbf{b}, (\mathbf{s}_1, \mathbf{X}_1), \dots, (\mathbf{s}_k, \mathbf{X}_k)) \overset{def}{=} \\
\textsc{GetValues}(\mathbf{R}_{\mathbf{Z}}^{-1}(\mathbf{R}_{\mathbf{Z}}(\mathcal{M})_{\mathbf{I} \leftarrow \mathbf{i}}), \mathbf{Outputs}).
\end{multline*}
\end{definition}

\input{tables/eq-results.tex}

\subsection{\Methodname}\label{sec:d-iit-obj}
Previous causal abstraction analyses of neural networks have performed brute-force search through a discrete space of hand-picked alignments. In \methodname\ (DAS), we find an alignment between one or more high-level variables and disjoint sub-spaces (but not necessarily sub-sets) of a large neural representation. 
The dimensions that are targeted for interventions are fixed, but the content of those dimensions is determined by the orthogonal matrix, which can be learned. 


We can define a distributed interchange intervention training objective and  then use PyTorch parameterizations for the space of orthogonal matrices to optimize for the objective with stochastic gradient descent. Crucially, the low-level and high-level models are frozen during learning.

\begin{definition}{\textnormal{Distributed Interchange Intervention Training Objective}}
Suppose we have a low-level neural network $\mathcal{L}$ with low-level input settings $\mathbf{Inputs}_L$ and a high-level algorithm $\mathcal{H}$ and want to align intermediate high-level variables $X_1, \dots, X_n \in \mathbf{Vars}_H$ with $k_1, \dots, k_n$ dimensions of a neural representation $\mathbf{N}$ after being rotated by an orthogonal matrix $R_{\mathbf{N}}$. Define $\Pi_{X_1}$ to be the first $k_1$ neurons of $\mathcal{H}$, $\Pi_{X_2}$ to be the next $k_2$ neurons, and so on.\footnote{We assume $\sum_{j=1}^n k_j \leq |\mathbf{N}|$.} We define the following differentiable objective, where $R^{\theta}_{\mathbf{N}}$ is a learned orthogonal matrix:
\begin{multline*}
\sum_{\begin{tabular}{c}
      $\mathbf{b},\mathbf{s}_1,\dots, \mathbf{s}_k \in \mathbf{Inputs}_L$\\
      $X_1, \dots, X_k \in \mathbf{Vars}_H$\\
\end{tabular}
      }  \hspace{-10pt} \textsc{Loss}\biggl(\\
      \tau \big (\dintinv(\mathcal{L},R^{\theta}_{\mathbf{N}}, \mathbf{b}, (\mathbf{s}_1, \Pi_{X_1}) \dots, (\mathbf{s}_n, \Pi_{X_n}))\big ), \\
      \intinv(\mathcal{H}, \tau(\mathbf{b}), (\tau(\mathbf{s}_1),{X}_1), \dots, (\tau(\mathbf{s}_n), {X}_n)\biggl)
\end{multline*}
\end{definition}\label{def:trainobj}
While we still have discrete hyperparameters $(\mathbf{N}, k_1, \dots, k_n)$---the target population and the dimensions of the sub-spaces for each high-level variable---the remaining computation is stochastic gradient descent to determine what rotation maximizes the distributed \intaccmetricabbr\ between $\mathcal{L}$ and $\mathcal{N}$. 


==> previousintro.tex <==

When are representations in a neural model explained by those of a higher-level algorithm?
The theory of causal abstraction provides a mathematical framework for faithful and interpretable explanations of AI models \cite{geigericard} by defining the conditions under which a complex causal system (e.g., a deep learning model) \emph{implements} a simpler causal system (e.g., a symbolic algorithm). Causal abstraction analysis has been used to identify neural representations of semantic relations in natural language inference models \cite{Geiger-etal:2019,Geiger-etal-2020} and neural representations of propositional content in language models \cite{Li2021}. 
However these applications have found a \emph{localist} representation in which each high-level variable maps to a separate population of neurons; in this paper we extend to \emph{distributed} representations in which high-level variables can be spread across (overlapping) populations of neurons \cite{PDP1, PDP2}. 

The fundamental operation on a causal model is an \textit{intervention} that fixes some set of variables to particular values \cite{pearl,Spirtes}. In causal abstraction analysis, an \textit{interchange intervention} is a method where a neural network is provided a `base' input and sets of neurons are forced to take on the values they would have if a different `source' input were provided. \citet{Geiger:2021} show that when a high-level causal model is aligned with representations in a neural network, the relevant causal abstraction relation holds when interchange interventions on aligned high-level variables and low-level variables have equivalent effects. A graded notion of a faithful alignment can be quantified with \textit{interchange intervention accuracy} (\intaccmetricabbr), which is the proportion of aligned interchange interventions with the same effect \cite{Geiger:2021}.

Previous applications of causal abstraction to model interpretation faced two central challenges: (1) They required a computationally intensive brute-force search process to find optimal alignments, and (2) they presupposed that high-level causal variables would be aligned with disjoint groups of neurons (i.e.~\textit{localist} representations). In this paper, we extend causal abstraction analysis to align interpretable high-level variables with overlapping low-level patterns \cite{Smolensky1986} in groups of neurons---\textit{distributed} neural representations.
In \methodname\ (\methodabbr), we learn best distributed representations to align to by gradient descent. Our key insight is that distributed representations are localist in an alternative basis (that is not aligned with individual neurons).
This procedure finds a distributed representation, and does so more efficiently than the brute-force search previously used to find localist representations. 












==> toyexample.tex <==
\begin{figure*}[p]
\centering
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \resizebox{\textwidth}{!}{
          \begin{tabular}{c c}
    \scriptsize$\mathbf{N} \overset{def}{=} \{H_{1,1},H_{1,2},H_{1,3},H_{1,4} \}$ &  \scriptsize $R_{\mathbf{N}} \overset{def}{=} \begin{bmatrix}
1/\sqrt{2} & \phantom{-}1/\sqrt{2} & 0 & 0 \\
1/\sqrt{2} & -1/\sqrt{2} & 0 & 0\\
   0  &  0 & \phantom{-}1/\sqrt{2} & 1/\sqrt{2} \\
    0 &  0 & -1/\sqrt{2} & 1/\sqrt{2} \\
\end{bmatrix}$\end{tabular} 
}
\vspace{15pt}
         \resizebox{\textwidth}{!}{
$\mathcal{N}(\begin{bmatrix}x_1 \\x_2\\ x_3\\x_4 \end{bmatrix}) \overset{def}{=} \sigma\Biggl(\ReLU\biggl(\ReLU\Bigl( \begin{bmatrix}x_1 \\x_2\\ x_3\\x_4 \end{bmatrix}^\text{T} \begin{bmatrix} \phantom{-}1 & -1 & \phantom{-}0 & \phantom{-}0 \\
-1 & \phantom{-}1 & \phantom{-}0 & \phantom{-}0\\
\phantom{-}0 & \phantom{-}0 & \phantom{-}1 & -1 \\
 \phantom{-}0 & \phantom{-}0 & -1 & \phantom{-}1 \\
\end{bmatrix}\Bigl)\begin{bmatrix} \phantom{-}1 & -1 & \phantom{-}0 & \phantom{-}1 \\
\phantom{-}1 & -1 & \phantom{-}0 & \phantom{-}1\\
-1 & \phantom{-}1 & \phantom{-}1 & \phantom{-}0 \\
 -1 & \phantom{-}1 & \phantom{-}1 & \phantom{-}0 \\
\end{bmatrix}\biggl) \begin{bmatrix} -1 \\ -1\\ \phantom{-}0.5 \\ \phantom{-}0.5\\ \end{bmatrix}\Biggl)$
}
    \caption{A hand-designed neural network that performs the hierarchical equality task, $\mathcal{N}$, a set of causal variables representing the first layer of that network, $\mathbf{N}$, and a rotation matrix, $\mathbf{R}_{\mathbf{N}}$.}
    \label{fig:equalitymath}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.49\textwidth}
         \resizebox{\textwidth}{!}{
             \input{figures/premack/network}
             }
    \caption{A causal model $\mathcal{N}$ representing a hand-designed neural network $\mathcal{N}$ that perform the hierarchical equality task. All variables take on real values. The causal mechanisms are determined by the weights.}
    \label{fig:equalitynetwork}
     \end{subfigure}

    \begin{subfigure}[t]{0.48\textwidth}
    \centering
                  \resizebox{0.7\textwidth}{!}{ 
             \input{figures/premack/networksetting}}
    \caption{The total setting $\mathcal{N}(0.23,0.23,0.91,-0.09)$ where the random one-dimensional embeddings are provided to $\mathcal{N}$. The final output is less than $0.5$ and so the network correctly predicts \false.}
    \label{fig:equalitynetworkinput}
     \end{subfigure}
     \hfill
    \begin{subfigure}[t]{0.48\textwidth}
    \centering
                  \resizebox{0.7\textwidth}{!}{ 
             \input{figures/premack/rotatednetworkinput}}
    \caption{The total setting of the rotated causal model $R_{\mathbf{N}}(\mathcal{N})(0.23,0.23,0.91,-0.09)$.
}
    \label{fig:equalityrotatednetworkinput}
     \end{subfigure}

         \begin{subfigure}[t]{0.48\textwidth}
    \centering
                  \resizebox{0.8\textwidth}{!}{ 
             \input{figures/premack/rotatednetworkintervention}}
    \caption{The total setting for an intervention on a rotated model\\ $R_{\mathbf{N}}(\mathcal{N})_{H_{(1,2)}\leftarrow 0 }(0.23,0.23,0.91,-0.09)$.}
    \label{fig:equalityrotatednetworkintervention}
     \end{subfigure}
     \hfill
    \begin{subfigure}[t]{0.48\textwidth}
    \centering
                  \resizebox{0.8\textwidth}{!}{ 
             \input{figures/premack/networkrotatedintervention}}
    \caption{The total setting for a distributed intervention \\ \centering $R_{\mathbf{N}}^{-1}(R_{\mathbf{N}}(\mathcal{N})_{H_{(1,2)} \leftarrow 0 })(0.23,0.23,0.91,-0.09)$.}
    \label{fig:equalitynetworkrotatedintervention}
     \end{subfigure}

\begin{subfigure}[t]{\textwidth}  
\centering
                  \resizebox{\textwidth}{!}{ 
\input{figures/BigMainFig.tex}
}
\caption{The distributed interchange intervention performed by rotating with $\mathbf{R}_{\mathbf{N}}$, interchange intervening, and unrotating with $\mathbf{R}_{\mathbf{N}}^T$, 
$\dintinv(\mathcal{N}$, 
$\mathbf{R}_{\mathbf{N}}$,
$[0.23,0.23,0.91,-0.09]$, 
$([0.91,0.23,-0.09,0.23], \{H_{(1,1)},H_{(1,2)}\})$, 
$([0.23,0.23,0.91,-0.09]  \{H_{(1,3)},H_{(1,4)}\}))$.}
\label{fig:equalityinterchange}
\end{subfigure}

    \caption{Causal models of a neural network that solve hierarchical equality.  Observe that rotating the first layer of the total settings from Figure~\ref{fig:equalitynetworkinput} and \ref{fig:equalitynetworkrotatedintervention} with the matrix $R_{\mathbf{N}}$ results in the total settings from Figure~\ref{fig:equalityrotatednetworkinput} and \ref{fig:equalitynetworkrotatedintervention}, respectively.}
        \label{fig:equality}
     
\end{figure*}


To further reinforce our empirical analysis of the hierarchical equality task (Section~\ref{sec:equality}), we consider a toy network $\mathcal{N}$ for the task, with handcrafted weights (Fig.~\ref{fig:equalitymath}). This network perfectly solves the task by implementing the algorithm with localist neural representations. Specifically, this network (1) computes whether the first pair of inputs are equal, storing the result in two left-most neurons of the first hidden layer, (2) computes whether the second pair of inputs are equal, storing the result in the two right-most neurons of the first hidden layer, and (3) computes whether these two representations encode the same truth-value. 

The localist alignment of the two intermediate variables of $\mathcal{A}$ with the first and second halves of the first layer of neurons achieves 100\% \intaccmetricabbr. An interchange intervention using this alignment is depicted in Fig.~\ref{fig:abstraction}.

However, there are also distributed alignments that achieve a perfect abstraction. For instance, if we rotate the layer of neurons $\mathbf{N}$ with orthogonal matrix $\mathbf{R}_{\mathbf{N}}$ defined in Figure~\ref{fig:equalitymath}, the same alignment works in this basis. This is because the orthogonal matrix does not entangle the first two dimensions with the second two dimensions, so the representations of simple equality relations are still disjoint under this new basis.

In Figure~\ref{fig:equalitynetwork}, we define the causal model $\mathcal{N}$ that represents the neural network analytically handcrafted to implement~$\mathcal{A}$. The four input variables take on the random real-values that represent each shape. The intermediate variables take on real-values and the output variable takes on a value between $0$ and $1$, with the network predicting $\true$ when the output is greater or equal to $0.5$, and $\false$ otherwise. The causal mechanisms of the intermediate and output variables are defined by the network weights.

To demonstrate the rotation operation, in Figure~\ref{fig:equalitynetworkinput} we depict the total setting of the network $\mathcal{N}$ when processing the input $[0.23,0.23,0.91,-0.09]$ and in Figure~\ref{fig:equalityrotatednetworkinput} we depict the network processing the same input, except the four neurons in the first layer are rotated by the orthogonal matrix~$\mathbf{R}_{\mathbf{N}}$.

To demonstrate a distributed intervention, in Figure~\ref{fig:equalitynetworkrotatedintervention}, we depict a distributed intervention on $\mathcal{N}$ where the first layer is rotated with $\mathbf{R}_{\mathbf{N}}$, the third neuron is fixed to be 0, then the first layer is unrotated with $\mathbf{R}_{\mathbf{N}}^{-1}$. In Figure~\ref{fig:equalityrotatednetworkintervention}, we depict the network before final rotation with $\mathbf{R}_{\mathbf{N}}^{-1}$.

Finally, in Figure~\ref{fig:equalityinterchange}, we depict a distributed interchange intervention with two intervention sites and source inputs. The first layer is rotated by $\mathbf{R}_{\mathbf{N}}$, then the interchange intervention is performed, then the first layer is unrotated by $\mathbf{R}_{\mathbf{N}}^T$. The two neural representations of simple equality relations would encode the values $(\true, \true)$ given the base input $[0.91,0.91,-0.09,-0.09]$, but instead are fixed to be values encoding $(\false, \false)$. 
\begin{figure*}[t!]
    \centering
\begin{subfigure}{0.96\textwidth}
    \centering
    
  \resizebox{0.7\textwidth}{!}{
    \input{figures/premack/Alignment}
    }
\begin{center}
\begin{tabular}{cccc}
    $\Pi_{O} = \{O_{\texttt{True}}\} $& $\Pi_{V_1} = \{H_{(1,1)}, H_{(1,2)}\}$ & $ \Pi_{V_2} = \{H_{(1,3)}, H_{(1,4)}\}$ & $\Pi_{I_j} = \{X_j\} \textnormal{ for } 1 \leq j \leq 4$ \\
\end{tabular}

\vspace{5pt}

\begin{tabular}{cc}
    $\tau_{O}(o_{\true}) = \begin{cases} \true & o_{\true} \geq 0.5 \\ \false & o_{\false} < 0.5 \\ \end{cases}$ & $\tau_{V_1}(h_{(1,1)}, h_{(1,2)}) = \begin{cases} \true & h_{(1,1)} = h_{(1,2)} = 0 \\ \false & \textnormal{Otherwise} \end{cases}$ \\[12pt]
      $\tau_{I_j}(x_j) = \begin{cases} \pentagon & x_j = 0.23\\ \square & x_j = 0.91 \\ \triangle & x_j = -0.11 \\ \end{cases}$ & $\tau_{V_2}(h_{(1,3)}, h_{(1,4)}) = \begin{cases} \true & h_{(1,3)} = h_{(1,4)} = 0 \\ \false & \textnormal{Otherwise} \end{cases}$ \\
\end{tabular}
\end{center}
    \caption{An alignment between the neural network $\mathcal{N}$ (left) and the symbolic algorithm $\mathcal{A}$ (right). The interchange intervention accuracy for this alignment is 100\%. An example of the algorithm $\mathcal{A}$ and the network $\mathcal{N}$ agreeing on an interchange intervention is shown in Figure~\ref{fig:interchangeintervention}.}
    \label{fig:alignment}
\end{subfigure}
\begin{subfigure}{0.96\textwidth}
    \centering
                              \resizebox{0.8\textwidth}{!}{ 
    \input{figures/InterchangeIntervention}
    }
    \caption{A single source interchange intervention where the counterfactual prediction of the network (bottom) agrees with the counterfactual prediction of the algorithm (top). We write this formally as\\ $[\tau \big (\intinv(\mathcal{A}, (\pentagon, \pentagon, \triangle, \square), (\square, \pentagon, \triangle, \triangle), V_2)\big ) = \intinv(\mathcal{N}, \tau(\pentagon, \pentagon, \triangle, \square), \tau(\square, \pentagon, \triangle, \triangle), \Pi_{V_2})]$.  }
    \label{fig:interchangeintervention}
\end{subfigure}

    \caption{An illustration of interchange intervention with the hierarchical equality task.}
    \label{fig:abstraction}
\end{figure*}

